Fine-grained Temporal Contrastive Learning for Weakly-supervised Temporal Action Localization

We target at the task of weakly-supervised action localization (WSAL), where only video-level action labels are available during model training. Despite the recent progress, existing methods mainly embrace a localization-by-classification paradigm and overlook the fruitful fine-grained temporal distinctions between video sequences, thus suffering from severe ambiguity in classification learning and classification-to-localization adaption. This paper argues that learning by contextually comparing sequence-to-sequence distinctions offers an essential inductive bias in WSAL and helps identify coherent action instances. Specifically, under a differentiable dynamic programming formulation, two complementary contrastive objectives are designed, including Fine-grained Sequence Distance (FSD) contrasting and Longest Common Subsequence (LCS) contrasting, where the first one considers the relations of various action/background proposals by using match, insert, and delete operators and the second one mines the longest common subsequences between two videos. Both contrasting modules can enhance each other and jointly enjoy the merits of discriminative action-background separation and alleviated task gap between classification and localization. Extensive experiments show that our method achieves state-of-the-art performance on two popular benchmarks. Our code is available at https://github.com/MengyuanChen21/CVPR2022-FTCL.

==> expr_tmp.tex <==
\subsection{Further Remarks}\label{sec:ablation}
To better understand our algorithm, we conduct ablation studies and in-depth analysis on the THUMOS14 dataset.


\noindent\textbf{Effectiveness of FSD Contrasting.}  In our proposed framework, we utilize FSD contrasting for discriminative foreground-background separation. To evaluate the effectiveness of this type of contrasting, we wipe out this module (denoted as FTCL(w/o FSD)) from the full model and observe a significant decrease in performance, as shown in~\tabref{}. Specifically, our full model FTCL outperforms the baseline by relative gains of ($x\%$, $x\%$, $x\%$,) on the XXX metrics. Without the FSD contrasting, fine-grained foreground-background distinctions can not be well handled, leading to insufficient classifier learning.


\noindent\textbf{Effectiveness of LCS Contrasting.}  We also remove LCS contrasting from the full model 
(FTCL(w/o LCS))) to evaluate its contribution to the overall perfromance, and the corresponding performance consistently drops as shown in~\tabref{}, proving the positive impact for robust classification-to-localization adaption. Note that mining LCS for untrimmed videos enables the model to discover coherent snippets in an action instance, thus facilitating the localization performance.


\noindent\textbf{Are the Above Two Modules Redundant?} Both the FSD and LCS objectives are adopted for sequence-to-sequence contrast but with different goals. Astute readers may be curious about whether the FSD and LCS learning strategies are redundant, \ie, could adopt either FSD or LCS for jointly modeling the foreground-background separation and classification-to-localization adaption? To answer this question, we conduct experiments with only FSD or LCS contrasting for tackling both the separation and adaption objectives, namely FTCL(both-FSD) and FTCL(both-LCS) in~\tabref{}. We can observe that our full model outperforms the two baselines, proving that the above two modules are not redundant. Another observation is that the both variants achieves better performance than FTCL(w/o FSD)) and FTCL(w/o LCS)). The reason lie in that both FSD and LCS belong to the sequence-to-sequence measurement, which can promote the separation and adaption objectives solely. However, since the two objectives have their unique properties, we desing the FSD and LCS contrasting strategy for respectively address them, which obtains the best performance.


\noindent\textbf{Why Not Resort to other Dynamic Programming Strategies like DTW?} We observe that there are some recent works pursuing the video sequence alignment based one dynamic time warping (DTW)~\cite{hadji2021representation,cao2020few,dvornik2021drop}. However, DTW assumes that the two sequences can be fully aligned, thus requiring trimmed videos. To validate the effectiveness of our FTCL, as shown in~\tabref{}, we compare our proposed method with the current state-of-the-art DTW-based approaches, Cycle-Consistency DTW (CC-DTW)~\cite{hadji2021representation} and  Drop-DTW~\cite{dvornik2021drop}. The results consistently demonstrate the superiority of our framework. We also replace our FSD and LCS strategies with the standard differentiable DTW operator~\cite{hadji2021representation} (detonted as DTW), which obtains inferior results as we analyzed above.


\noindent\textbf{Complementary Role of the proposed FTCL.} It is obvious that the proposed strategy is model-agnostic and non-intrusive, and hence can play a complementary role over existing methods. In~\tabref{}, we plug our FSD and LCS contrasting into four WSAL approaches including STPN~\cite{}, W-TALC~\cite{}, CoLA~\cite{}, and FAC-Net~\cite{}. The results shows that our proposed learning strategies can consistently improve their performance. In addition, our method does not introduce computational cost during model inference. Note that CoLA also adopts contrastive learning in the snippet-level, our proposed method can further boost its performance by additionally considering the fine-grained temporal distinctions.


\noindent\textbf{Other Ablation studies.}
Please refer to \textbf{Supplementary Material} for other ablations, such as the threshold $\tau$, feature analysis via t-SNE visualization, different ranking loss $\ell(x)$, and the balance term $\lambda$,~\etc. 

\subsection{Qualitative Results}\label{sec:qualitative}
To interpret how our framework can utilize fine-grained temproal distinctions between differnt videos, \figref{} illustrates the aligned snippets between two videos from the same action category \emph{XXX} by using the learned LCS recursion matrix. From this figure we can observe that XXX. 


